Making Attention Mechanisms More Robust and Interpretable with Virtual Adversarial Training

Although attention mechanisms have become fundamental components of deep learning models, they are vulnerable to perturbations, which may degrade the prediction performance and model interpretability. Adversarial training (AT) for attention mechanisms has successfully reduced such drawbacks by considering adversarial perturbations. However, this technique requires label information, and thus, its use is limited to supervised settings. In this study, we explore the concept of incorporating virtual AT (VAT) into the attention mechanisms, by which adversarial perturbations can be computed even from unlabeled data. To realize this approach, we propose two general training techniques, namely VAT for attention mechanisms (Attention VAT) and "interpretable" VAT for attention mechanisms (Attention iVAT), which extend AT for attention mechanisms to a semi-supervised setting. In particular, Attention iVAT focuses on the differences in attention; thus, it can efficiently learn clearer attention and improve model interpretability, even with unlabeled data. Empirical experiments based on six public datasets revealed that our techniques provide better prediction performance than conventional AT-based as well as VAT-based techniques, and stronger agreement with evidence that is provided by humans in detecting important words in sentences. Moreover, our proposal offers these advantages without needing to add the careful selection of unlabeled data. That is, even if the model using our VAT-based technique is trained on unlabeled data from a source other than the target task, both the prediction performance and model interpretability can be improved.

==> images/tex/loss_supervised.tex <==
\begin{figure*}[t]
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig_loss_SST.pdf}
        \subcaption{SST}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig_loss_IMDB.pdf}
        \subcaption{IMDB}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig_loss_CNN.pdf}
        \subcaption{CNN news}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig_loss_Multi_NLI.pdf}
        \subcaption{MultiNLI}
    \end{minipage}
    \caption{Learning curves for single sequence tasks (SST and IMDB), and pair sequence tasks (CNN news and MultiNLI) in supervised settings. We show the transition of loss (defined in Eq.~\ref{eq:overall_loss}) on the validation sets. For all four tasks, we can observe that our Attention VAT/iVAT prevents overfitting better than the vanilla model and even Word VAT/iVAT models. This advantage is more significant in the pair sequence tasks.}
    \label{fig:loss_supervised}
\end{figure*}

==> tables/tex/classification_score/010_supervised.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of \textit{supervised} prediction performance and the Pearson's correlation coefficients (Corr.) between the attention weight and the word importance of the gradient-based method in both supervised models. 
The training data for the pair sequence task is half of the original training data.
}
\label{tab:supervised_score}
\begin{minipage}{\linewidth}
    \subcaption{Single sequence task}
    \centering
    \resizebox{\textwidth}{!}{%
    \input{tables/tex/classification_score/011_supervised_single_sequence}
    }
\end{minipage}

\begin{minipage}{\linewidth}
    \subcaption{Pair sequence task}
    \centering
    \resizebox{\textwidth}{!}{%
    \input{tables/tex/classification_score/012_supervised_pair_sequence}
    }
\end{minipage}
\end{table*}

==> tables/tex/classification_score/011_supervised_single_sequence.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SST\\ $N_l$ = 6,920\end{tabular}}                                 & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}IMDB\\ $N_l$ = 17,186\end{tabular}}                                & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}20News\\ $N_l$ = 1,145\end{tabular}}                              & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}AGNews\\ $N_l$ = 51,000\end{tabular}}                              \\ \cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{F1 [\%]} & \multicolumn{1}{c}{Corr.} & \multicolumn{1}{c}{F1 [\%]} & \multicolumn{1}{c}{Corr.} & \multicolumn{1}{c}{F1 [\%]} & \multicolumn{1}{c}{Corr.} & \multicolumn{1}{c}{F1 [\%]} & \multicolumn{1}{c}{Corr.} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Vanilla~\cite{jain2019attention}            & 79.27                       & 0.852                     & 88.77                       & 0.788                     & 95.05                       & 0.891                     & 95.27                       & 0.822                     \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Word AT~\cite{miyato2016adversarial}       & 79.61                       & 0.647                     & 89.65                       & 0.838                     & 95.11                       & 0.892                     & 95.59                       & 0.813                     \\
Word iAT~\cite{sato2018interpretable}      & 79.57                       & 0.643                     & 89.64                       & 0.839                     & 95.14                       & 0.893                     & 95.62                       & 0.809                     \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Word VAT~\cite{miyato2018virtual}          & 81.90                       & 0.651                     & 89.79                       & 0.841                     & 96.32                       & 0.903                     & 95.98                       & 0.817                     \\
Word iVAT~\cite{sato2018interpretable}     & 81.98                       & 0.648                     & 89.78                       & 0.843                     & 96.30                       & 0.907                     & 96.01                       & 0.814                     \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention AT~\cite{kitada2021attention}    & 81.72                       & 0.852                     & 90.00                       & 0.819                     & 96.69                       & 0.868                     & 96.12                       & 0.835                     \\
Attention iAT~\cite{kitada2021attention}   & 82.20                       & 0.876                     & \textbf{90.21}              & \textbf{0.861}            & 96.58                       & 0.897                     & 96.19                       & 0.891                     \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention VAT (\textbf{Proposed})              & 82.19                       & 0.878                     & 90.20                       & 0.859                     & \textbf{96.71}              & \textbf{0.913}            & 96.18                       & 0.888                     \\
Attention iVAT (\textbf{Proposed})             & \textbf{82.21}              & \textbf{0.881}            & 90.18                       & 0.857                     & 96.70                       & 0.909                     & \textbf{96.21}              & \textbf{0.897}            \\ \bottomrule
\end{tabular}

==> tables/tex/classification_score/012_supervised_pair_sequence.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{Model}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}CNN news\\ $N_l$ = 190,149\end{tabular}}     & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SNLI\\ $N_l$ = 274,683\end{tabular}}              & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}MultiNLI\\ $N_l$ = 157,080\end{tabular}}                                              \\ \cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-9}
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{\multirow{2}{*}{Acc. [\%]}} & \multicolumn{1}{c}{\multirow{2}{*}{Corr.}} & \multicolumn{1}{c}{\multirow{2}{*}{Micro-F1 [\%]}} & \multicolumn{1}{c}{\multirow{2}{*}{Corr.}} & \multicolumn{3}{c}{Micro-F1 [\%]}                                                       & \multicolumn{1}{c}{\multirow{2}{*}{Corr.}} \\ \cmidrule(lr){6-8}
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                               & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{Avg.} & \multicolumn{1}{c}{Matched} & \multicolumn{1}{c}{Mismatched} & \multicolumn{1}{c}{}                       \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Vanilla~\cite{jain2019attention}           & 56.25                                          & 0.638                                      & 73.52                                              & 0.741                                      & 56.59                    & 56.65                       & 56.53                          & 0.517                                      \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Word AT~\cite{miyato2016adversarial}       & 60.87                                          & 0.691                                      & 75.85                                              & 0.757                                      & 57.82                    & 57.99                       & 57.65                          & 0.574                                      \\
Word iAT~\cite{sato2018interpretable}      & 61.21                                          & 0.702                                      & 75.91                                              & 0.758                                      & 57.91                    & 58.01                       & 57.81                          & 0.581                                      \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Word VAT~\cite{miyato2018virtual}          & 61.79                                          & 0.692                                      & 76.01                                              & 0.761                                      & 57.89                    & 58.05                       & 57.73                          & 0.598                                      \\
Word iVAT~\cite{sato2018interpretable}     & 61.89                                          & 0.698                                      & 76.42                                              & 0.767                                      & 58.02                    & 58.07                       & 57.97                          & 0.595                                      \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention AT~\cite{kitada2021attention}    & 62.08                                          & 0.742                                      & 77.21                                              & 0.769                                      & 59.28                    & 59.45                       & 59.11                          & 0.593                                      \\
Attention iAT~\cite{kitada2021attention}   & \textbf{62.15}                                 & \textbf{0.753}                             & 77.23                                              & 0.772                                      & 59.42                    & 59.54                       & 59.25                          & 0.622                                      \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention VAT (\textbf{Proposed})          & 62.05                                          & 0.739                                      & 77.22                                              & 0.779                                      & 59.37                    & 59.47                       & 59.27                          & 0.621                                      \\
Attention iVAT (\textbf{Proposed})         & 62.12                                          & 0.744                                      & \textbf{77.27}                                     & \textbf{0.781}                             & \textbf{59.43}           & \textbf{59.55}              & \textbf{59.31}                 & \textbf{0.623}                             \\ \bottomrule
\end{tabular}

==> tables/tex/classification_score/020_semi_supervised.tex <==
\begin{table*}[t]
\centering
\caption{
Comparison of \textit{semi-supervised} prediction performance and the Pearson's correlation coefficients (Corr.) between the attention weight and the word importance of the gradient-based method. 
The value $N_{u}$ stands for the number of unlabeled examples in the training set and is determined with validation performance.
In the single sequence tasks, we use randomly selected sentences from unlabeled data pool without special selection to be added.
On the other hand, in the pair sequence task, half of each dataset is used as unlabeled data because external sentences cannot be used due to the nature of the task.
}
\label{tab:semi_supervised_score}
\begin{minipage}{\linewidth}
    \subcaption{Single sequence task}
    \centering
    \resizebox{\textwidth}{!}{%
    \input{tables/tex/classification_score/021_semi_supervised_single_seqnece}
    }
\end{minipage}

\begin{minipage}{\linewidth}
    \subcaption{Pair sequence task}
    \centering
    \resizebox{\textwidth}{!}{%
    \input{tables/tex/classification_score/022_semi_supervised_pair_sequence}
    }
\end{minipage}
\end{table*}

==> tables/tex/classification_score/021_semi_supervised_single_seqnece.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SST\\ $N_u$ = 50,000\\ $N_u/N_l$ = 7.22\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}IMDB\\ $N_u$ = 150,000\\$N_u/N_l$ = 8.23\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}20News\\ $N_u$ = 25,000\\$N_l/N_u$ = 21.83\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}AGNews\\ $N_u$ = 250,000\\ $N_u/N_l$ = 4.90\end{tabular}} \\ \cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{F1 [\%]}                    & \multicolumn{1}{c}{Corr.}                   & \multicolumn{1}{c}{F1 [\%]}                     & \multicolumn{1}{c}{Corr.}                    & \multicolumn{1}{c}{F1 [\%]}                     & \multicolumn{1}{c}{Corr.}                     & \multicolumn{1}{c}{F1 [\%]}                      & \multicolumn{1}{c}{Corr.}                     \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Word VAT~\cite{miyato2018virtual}          & 83.04                                          & 0.779                                       & 92.21                                           & 0.853                                        & 96.79                                           & 0.908                                         & 96.23                                            & 0.831                                         \\
Word iVAT~\cite{sato2018interpretable}     & 83.07                                          & 0.781                                       & 92.30                                           & 0.859                                        & 96.73                                           & 0.911                                         & 96.17                                            & 0.827                                         \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention VAT (\textbf{Proposed})              & 83.18                                          & 0.898                                       & 92.48                                           & 0.879                                        & \textbf{96.98}                                  & \textbf{0.918}                                & 96.35                                            & 0.903                                         \\
Attention iVAT (\textbf{Proposed})             & \textbf{83.22}                                 & \textbf{0.901}                              & \textbf{92.56}                                  & \textbf{0.883}                               & 96.93                                           & 0.916                                         & \textbf{96.48}                                   & \textbf{0.917}                                \\ \bottomrule
\end{tabular}

==> tables/tex/classification_score/022_semi_supervised_pair_sequence.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{Model}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}CNN news\\ $N_u$ = 190,149\\ $N_u/N_l = $ 1.00\end{tabular}}      & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SNLI\\ $N_u$ = 274,683\\ $N_u/N_l = $ 1.00\end{tabular}}              & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}MultiNLI\\ $N_u$ = 157,081\\ $N_u/N_l = $ 1.00\end{tabular}}                                              \\ \cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-9}
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{\multirow{2}{*}{Acc. [\%]}} & \multicolumn{1}{c}{\multirow{2}{*}{Corr.}} & \multicolumn{1}{c}{\multirow{2}{*}{Micro-F1 [\%]}} & \multicolumn{1}{c}{\multirow{2}{*}{Corr.}} & \multicolumn{3}{c}{Micro-F1 [\%]}                                                       & \multicolumn{1}{c}{\multirow{2}{*}{Corr.}} \\ \cmidrule(lr){6-8}
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                           & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                               & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{Avg.} & \multicolumn{1}{c}{Matched} & \multicolumn{1}{c}{Mismatched} & \multicolumn{1}{c}{}                       \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Word VAT~\cite{miyato2018virtual}          & 63.74                                          & 0.749                                      & 77.38                                              & 0.758                                      & 60.43                    & 60.57                       & 60.29                          & 0.629                                      \\
Word iVAT~\cite{sato2018interpretable}     & 63.76                                          & 0.751                                      & 77.42                                              & 0.761                                      & 60.47                    & 60.62                       & 60.32                          & 0.631                                      \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention VAT (\textbf{Proposed})          & 64.93                                          & 0.766                                      & 77.87                                              & 0.784                                      & 61.07                    & 61.11                       & 61.03                          & 0.638                                      \\
Attention iVAT (\textbf{Proposed})         & \textbf{65.08}                                 & \textbf{0.773}                             & \textbf{78.13}                                     & \textbf{0.808}                             & \textbf{61.18}           & \textbf{61.22}              & \textbf{61.14}                 & \textbf{0.647}                             \\ \bottomrule
\end{tabular}

==> tables/tex/classification_score/031_semi_supervised_random.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SST\\ $N_{u}$ = 50,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}IMDB\\ $N_{u}$ = 150,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}20News\\ $N_{u}$ = 25,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}AGNews\\ $N_{u}$ = 250,000\end{tabular}} \\ \cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9}
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{F1 [\%]}                    & \multicolumn{1}{c}{Corr.}                   & \multicolumn{1}{c}{F1 [\%]}                     & \multicolumn{1}{c}{Corr.}                    & \multicolumn{1}{c}{F1 [\%]}                     & \multicolumn{1}{c}{Corr.}                     & \multicolumn{1}{c}{F1 [\%]}                      & \multicolumn{1}{c}{Corr.}                     \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention VAT (\textbf{Proposed})              & 83.18                                          & 0.898                                       & 92.48                                           & 0.879                                        & \textbf{96.98}                                  & \textbf{0.918}                                & 96.35                                            & 0.903                                         \\
Attention iVAT (\textbf{Proposed})             & \textbf{83.22}                                 & \textbf{0.901}                              & \textbf{92.56}                                  & \textbf{0.883}                               & 96.93                                           & 0.916                                         & \textbf{96.48}                                   & \textbf{0.917}                                \\ \bottomrule
\end{tabular}

==> tables/tex/classification_score/032_semi_supervised_BoW.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SST\\ $N_u$ = 50,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}IMDB\\ $N_u $= 150,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}20News\\ $N_u$ = 25,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}AGNews\\ $N_u$ = 250,000\end{tabular}} \\ \cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{F1 [\%]}              & \multicolumn{1}{c}{Corr.}             & \multicolumn{1}{c}{F1 [\%]}               & \multicolumn{1}{c}{Corr.}              & \multicolumn{1}{c}{F1 [\%]}               & \multicolumn{1}{c}{Corr.}               & \multicolumn{1}{c}{F1 [\%]}                & \multicolumn{1}{c}{Corr.}               \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention VAT (\textbf{Proposed})              & 83.20                                    & 0.903                                 & 92.51                                     & 0.884                                  & \textbf{97.01}                            & \textbf{0.924}                          & 96.38                                      & 0.908                                   \\
Attention iVAT (\textbf{Proposed})             & \textbf{83.26}                           & \textbf{0.909}                        & \textbf{92.59}                            & \textbf{0.891}                         & 96.97                                     & 0.924                                   & \textbf{96.51}                             & \textbf{0.924}                          \\ \bottomrule
\end{tabular}

==> tables/tex/classification_score/033_semi_supervised_Avg_W2V.tex <==
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SST\\ $N_u$ = 50,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}IMDB\\ $N_u $= 150,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}20News\\ $N_u$ = 25,000\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}AGNews\\ $N_u$ = 250,000\end{tabular}} \\ \cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{F1 [\%]}              & \multicolumn{1}{c}{Corr.}             & \multicolumn{1}{c}{F1 [\%]}               & \multicolumn{1}{c}{Corr.}              & \multicolumn{1}{c}{F1 [\%]}               & \multicolumn{1}{c}{Corr.}               & \multicolumn{1}{c}{F1 [\%]}                & \multicolumn{1}{c}{Corr.}               \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} \cmidrule(lr){8-8} \cmidrule(l){9-9}
Attention VAT (\textbf{Proposed})              & 83.21                                    & 0.927                                 & 92.50                                     & 0.902                                  & 96.96                                     & 0.948                                   & 96.38                                      & 0.928                                   \\
Attention iVAT (\textbf{Proposed})             & \textbf{83.26}                           & \textbf{0.941}                        & \textbf{92.60}                            & \textbf{0.914}                         & \textbf{97.00}                            & \textbf{0.953}                          & \textbf{96.51}                             & \textbf{0.957}                          \\ \bottomrule
\end{tabular}
